Deep Learning Innovations for Underwater Waste Detection: An In-Depth Analysis

Addressing the issue of submerged underwater trash is crucial for safeguarding aquatic ecosystems and preserving marine life. While identifying debris present on the surface of water bodies is straightforward, assessing the underwater submerged waste is a challenge due to the image distortions caused by factors such as light refraction, absorption, suspended particles, color shifts, and occlusion. This paper conducts a comprehensive review of state-of-the-art architectures and on the existing datasets to establish a baseline for submerged waste and trash detection. The primary goal remains to establish the benchmark of the object localization techniques to be leveraged by advanced underwater sensors and autonomous underwater vehicles. The ultimate objective is to explore the underwater environment, to identify, and remove underwater debris. The absence of benchmarks (dataset or algorithm) in many researches emphasizes the need for a more robust algorithmic solution. Through this research, we aim to give performance comparative analysis of various underwater trash detection algorithms.

==> datatable.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
\begin{table}[h!]

\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
{\ul \textbf{Type}} &
  {\ul \textbf{Dataset}} &
  {\ul \textbf{Images}} &
  {\ul \textbf{Classes}} &
  {\ul \textbf{instances}} &
  {\ul \textbf{Environment}} &
  {\color[HTML]{2E2E2E} {\ul \textbf{Annotation type}}} \\ \hline
{\color[HTML]{2E2E2E} } &
  {\color[HTML]{2E2E2E} Open Litter Map} &
  {\color[HTML]{2E2E2E} \textgreater{}100 k} &
  {\color[HTML]{2E2E2E} \textgreater{}100} &
  {\color[HTML]{2E2E2E} \textgreater{}100 k} &
  {\color[HTML]{2E2E2E} outdoor} &
  {\color[HTML]{2E2E2E} multilabels} \\ \cline{2-7} 
{\color[HTML]{2E2E2E} } &
  {\color[HTML]{2E2E2E} TrashNet} &
  {\color[HTML]{2E2E2E} 2194} &
  {\color[HTML]{2E2E2E} 5} &
  {\color[HTML]{2E2E2E} 2194} &
  {\color[HTML]{2E2E2E} indoor} &
  {\color[HTML]{2E2E2E} labels} \\ \cline{2-7} 
{\color[HTML]{2E2E2E} } &
  {\color[HTML]{2E2E2E} Waste Pictures} &
  {\color[HTML]{2E2E2E} 23,633} &
  {\color[HTML]{2E2E2E} 34} &
  {\color[HTML]{2E2E2E} 23,633} &
  {\color[HTML]{2E2E2E} outdoor} &
  {\color[HTML]{2E2E2E} labels} \\ \cline{2-7} 
\multirow{{\color[HTML]{2E2E2E} \textit{\textbf{Classification}}}} &
  {\color[HTML]{2E2E2E} Places} &
  {\color[HTML]{2E2E2E} 2.5 M} &
  {\color[HTML]{2E2E2E} 205} &
  {\color[HTML]{2E2E2E} 2.5 M} &
  {\color[HTML]{2E2E2E} background} &
  {\color[HTML]{2E2E2E} labels} \\ \hline
{\color[HTML]{2E2E2E} } &
  {\color[HTML]{2E2E2E} Drinking waste} &
  {\color[HTML]{2E2E2E} 4810} &
  {\color[HTML]{2E2E2E} 4} &
  {\color[HTML]{2E2E2E} 5058} &
  {\color[HTML]{2E2E2E} indoor} &
  {\color[HTML]{2E2E2E} bounding box} \\ \cline{2-7} 
{\color[HTML]{2E2E2E} } &
  {\color[HTML]{2E2E2E} Extended TACO} &
  {\color[HTML]{2E2E2E} 4562} &
  {\color[HTML]{2E2E2E} 7} &
  {\color[HTML]{2E2E2E} 14,286} &
  {\color[HTML]{2E2E2E} outdoor} &
  {\color[HTML]{2E2E2E} bounding box} \\ \cline{2-7} 
{\color[HTML]{2E2E2E} } &
  {\color[HTML]{2E2E2E} MJU-Waste} &
  {\color[HTML]{2E2E2E} 2475} &
  {\color[HTML]{2E2E2E} 1} &
  {\color[HTML]{2E2E2E} 2532} &
  {\color[HTML]{2E2E2E} indoor} &
  {\color[HTML]{2E2E2E} instance masks} \\ \cline{2-7} 
{\color[HTML]{2E2E2E} } &
  {\color[HTML]{2E2E2E} TrashCan} &
  {\color[HTML]{2E2E2E} 7212} &
  {\color[HTML]{2E2E2E} 8} &
  {\color[HTML]{2E2E2E} 6214} &
  {\color[HTML]{2E2E2E} underwater} &
  {\color[HTML]{2E2E2E} instance masks} \\ \cline{2-7} 
{\color[HTML]{2E2E2E} } &
  {\color[HTML]{2E2E2E} Trash-ICRA} &
  {\color[HTML]{2E2E2E} 7668} &
  {\color[HTML]{2E2E2E} 7} &
  {\color[HTML]{2E2E2E} 6706} &
  {\color[HTML]{2E2E2E} underwater} &
  {\color[HTML]{2E2E2E} bounding box} \\ \cline{2-7} 
{\color[HTML]{2E2E2E} } &
  {\color[HTML]{2E2E2E} UAVVaste} &
  {\color[HTML]{2E2E2E} 772} &
  {\color[HTML]{2E2E2E} 1} &
  {\color[HTML]{2E2E2E} 3718} &
  {\color[HTML]{2E2E2E} outdoor} &
  {\color[HTML]{2E2E2E} instance masks} \\ \cline{2-7} 
\multirow{{\color[HTML]{2E2E2E} \textit{\textbf{Detection}}}} &
  {\color[HTML]{2E2E2E} Wade-AI} &
  {\color[HTML]{2E2E2E} 1396} &
  {\color[HTML]{2E2E2E} 1} &
  {\color[HTML]{2E2E2E} 2247} &
  {\color[HTML]{2E2E2E} outdoor} &
  {\color[HTML]{2E2E2E} instance masks} \\ \hline
\end{tabular}%

}
\caption{Table comparing existing public datasets}
\end{table}


==> related.tex <==
\subsection{Challenges in Marine Debris Detection }
The primary challenge stems from the relatively small size of debris compared to the ocean body, its submerged nature, and the potential for it to be concealed in the sea bottom. However, Moorton's \cite{028} paper provides a thoughtful query to the research community - is the use of deep learning to locate ocean debris potentially harmful to aquatic wildlife? Accurate visual and sensory detection of underwater litter using deep learning requires a substantial and well-labeled collection of underwater debris. \\

\subsection{Technological Approaches to Detection }


This review aims to provide an in-depth overview of object detection algorithms that utilize deep learning. 
\begin{figure}[h!]

\centering
  \includegraphics[width=1\linewidth]{image.png}
  \caption{Taxonomy for categorizing various contributions for deep learning-based object detection \cite{bigpaper}.
}

\end{figure}
Figure 1 \cite{bigpaper} outlines the primary object detection methodologies organizing the diverse contributions in deep learning-based object detection into three main categories: detection components, learning strategies, and applications \& benchmarks. 
Ongoing research focuses on the development of autonomous robot systems for studying natural aquatic environments, encompassing both surface and underwater levels. Moreover, numerous robotic systems have been proposed for environmental monitoring \cite{Girdhar2011MARE}, environmental mapping \cite{temp1}, and maritime robotics for guidance and localization \cite{Torrey2009Chapter1T, DREVER2018684, tftf, DERRAIK2002842}. \\
In their study on at-sea tracking of aquatic debris \cite{inproceedings}, Mace et al. explored various strategies and technological approaches for detecting underwater debris. \\
After the occurrence of the Japan tsunami in 2011, researchers explored methods to mitigate debris from the ocean's surface \cite{article1}. In a related context, Ge et al. \cite{17} utilized LIDAR technology to locate and document beach garbage. \\
The study titled "Sonar image garbage detection via global despeckling and dynamic attention graph optimization" \cite{18} introduces an innovative model tailored for sonar image garbage identification. \\
Additionally, the underwater image enhancement method with light scattering characteristics \cite{19} proposes a technique leveraging light scattering characteristics to enhance the quality of underwater images and thereby improve visibility. \\
Furthermore, the two-step domain adaptation for underwater image enhancement \cite{20} contributes to image enhancement techniques with a two-step adapted approach specifically designed for underwater images, potentially improving the efficiency of image-based debris detection algorithms. \\
Operational use of multispectral images for macro-litter mapping and categorization by Unmanned Aerial Vehicle \cite{22} explores the integration of drone technology and multispectral imaging to map and categorize large litter pieces. \\

\subsection{Deep Learning in Underwater Debris Detection }

Further adding to the pool of studies utilizing deep learning techniques for the detection of underwater debris, Kshirsagar \cite{018} discusses an approach that leverages image processing techniques for ocean pollution detection. \\
Deep learning paradigms are not only utilized for detection but also for enhancing image quality. Innovative research by Kylili \cite{022} capitalized on a deep learning approach to identify floating plastic marine debris. Bolstering the argument for deep learning-based debris detection, notable work by Xue \cite{025,026} and Bajaj \cite{027} presents efficacious methodologies to detect deep-sea debris, employing deep neural networks and offering valuable insights into underwater debris identification. Jian \cite{029} adopted a unique path by focusing on the reduction of haziness in a single underwater image, dovetailing with other research aimed at deep-learning image enhancement to improve debris detection accuracy. \\
Lastly, Alejandro \cite{030} and Zhou \cite{031} contribute to the research domain by experimenting with marine debris location and recognition using object detection, proposing a novel 'YOLOTrashCan' network for marine debris identification. \\
\subsection{Datasets and Environmental Impact }

Laibin Chang's study introduces the UIDEF dataset, a real-world collection of over 9000 diverse underwater images \cite{128}. The first report of deep-sea litter in the South-Western Caribbean Sea \cite{21} provides valuable insights into the presence and distribution of deep-sea litter in the specified region. \\
The BeachLitter dataset for image segmentation \cite{23} establishes a dedicated dataset for beach litter. For instance, the Monterey Bay Aquarium Research Institute, as reported in Environmental Science \& Technology, has been amassing data on ocean floor trash for over 22 years along the west coast of the USA, with a focus on metal and plastic debris in and around the Monterey Canyon \cite{4524846}. \\
Another noteworthy example is the dataset compiled by JAMSTEC (Global Oceanographic Data Center), a division of the Japan Agency for Maritime Earth Science and Technology \cite{tftf}. \\

\subsection{Environmental Conservation Efforts }

Clear Blue Sea, an altruistic community dedicated to environmental safeguarding and cleaning, has proposed the use of 'FRED (Floating Robot for Eliminating Debris)' cars\cite{Derraik2002ThePO}. \\
In a similar vein, The Rozalia Project, a non-profit organization, employs numerous underwater rovers equipped with multi-beam and side-scan sonars to detect debris in aquatic bodies\cite{88df61e7069a431085e274d3c9068466}. 

\subsection{Alternative Solutions and Innovations }

The National Oceanic and Atmospheric Administration (NOAA) has explored the possibility of monitoring marine environments by leveraging the identification of underwater biological occurrences \cite{NOAA}. Initiatives have also been undertaken to locate and examine marine debris and garbage, studying their dispersal patterns on the ocean's surface, particularly along eddy currents and other potential ocean currents. Similarly, Howell \cite{4524846} arrived at a parallel conclusion while investigating marine detritus, particularly focusing on abandoned fishing gear in the North Pacific Ocean region. Furthermore, autonomous debris detection and compilation in terrestrial settings were successfully evaluated, as seen in the work by Kulkarni et al. \cite{17}. Complementing this, Kaur \cite{019} explores quality improvement techniques for underwater images, focusing on species classification. \\

There have been many notable contributions of underwater debris detection models using deep learning in the recent years. Guo \cite{021} proposed an advanced technique that employs transformers\cite{101} for unsupervised underwater image enhancement followed by, Zhang's synthesis \cite{023} of image analysis methods for microorganism counting showcases the extensive applicability of deep learning in imaging used for underwater investigation. Fu \cite{024} advances this area further by comparing RFE-DL and stacking ensemble learning algorithms for classifying mangrove species on UAV multispectral images. Ivana Marin's work presents a deep-feature-based approach enhancing the accuracy and efficiency of marine debris classification \cite{129}. Frederieke J. Kroon investigates the classification of marine microdebris, offering a comprehensive analysis through a case study in the Great Barrier Reef \cite{130}. Marinella Farré explores the effective use of remote sensing and in-situ devices for marine debris detection \cite{131}. L. Fallati showcases the combined utilization of UAV imagery and deep learning for marine debris assessment along the beaches of the Republic of Maldives \cite{132}. \\

Manisha Vashisht's survey on object detection methods and another paper on image classification methods offer crucial overviews influencing strategies for underwater image classification and debris detection \cite{133,134}. Paula M.'s study provides insight into future prospects of using remote sensing for marine litter assessment, emphasizing advancements and aspirations \cite{135}. "A Survey of Deep Learning Techniques for Underwater Image Classification" by Sparsh Mittal \cite{27} provides a comprehensive review of various deep-learning techniques applied to underwater image classification. \\In a recent study by Valdenegro-Toro\cite{DBLP:journals/corr/abs-2108-06800}, a deep convolutional architecture designed for forward-looking-sonar (FLS) images demonstrated an 80\% accuracy in detecting aquatic detritus. Recent strides in underwater imaging and marine debris detection have been marked by significant advancements. Kylili's study introduced the Adaptive Lighting Enhancement (ALE) algorithm, crucial for enhancing image intensity and contrast in underwater conditions \cite{100}. \\
Highlighting the utility of machine learning in environmental conservation,  research ventured into identifying floating plastic marine debris using deep learning, achieving an 86\% accuracy in classifying objects such as bottles and straws \cite{102}. In 2022, researchers Kshirsagar et.al explored ocean pollution detection using advanced image processing, including color correction and histogram equalization \cite{103}. \\
Several publications also took a step further with training lightweight neural networks for deep-sea debris detection, utilizing the JAMSTEC dataset for training \cite{104} which couldnt erradicate the problem of bias-adaptation due to overfitting on one single type of dataset.

Apart from advancing in the deep learning technique, studies for haze removal in underwater images using linear learning models \cite{105} have been performed to make detection easier by pre-processing. Xue et.al performed deep-sea debris detection using ResNet50-YOLOv3 model tailored for AUV technology \cite{106} and a Hybrid Shuffle-Xception network for debris classification \cite{107} demonstrated the potential of deep learning in addressing these environmental challenges. Further exploring deep learning applications, \cite{108} discussed the use of the InceptionResNetV2 architecture for sea debris detection, while Moorton et.al also raised questions about the impact of these technologies on aquatic wildlife in his work \cite{109}.\\ 

In Pattern Recognition, using the CleanSea dataset \cite{110}, alongside the introduction of YOLOTrashCan for marine debris detection \cite{111}, indicates significant advancements in underwater object detection. Furthermore, the publication on UIDEF dataset and image enhancement \cite{112}, Mdpi's 2021 study on deep-feature-based marine debris classification \cite{113}, and further research in the field collectively contribute to the understanding and technological advancement in underwater image enhancement and marine debris detection. \\
